The Basic Theory of Clifford-Bianchi Groups for Hyperbolic n-Space

Let $K$ be a $\mathbb{Q}$-Clifford algebra associated to an $(n-1)$-ary positive definite quadratic form, and let $\mathcal{O}$ be a maximal order in $K$. For each such order we define a Clifford-Bianchi group $\operatorname{SL}_2(\mathcal{O})$, generalizing Bianchi groups associated to orders in imaginary quadratic fields. We study the arithmetic of maximal orders and the actions of these groups on hyperbolic space $\mathcal{H}^{n+1}$ by M\"obius transformations $x\mapsto (ax+b)(cx+d)^{-1}$. We develop the general theory of orders and exhibit explicit low-dimensional examples, including higher-dimensional analogues of the Hurwitz order and an order whose lattice of Clifford vectors is the $E_8$ lattice. We develop abstract and computational methods for determining fundamental domains, generators, and relations. The existence of these domains follows from a moduli interpretation extending Swan's Bianchi-Humbert theory; the domains do not follow from general considerations involving Siegel sets. We connect this theory to the classical literature on symmetric spaces and arithmetic groups, and prove that Clifford-Bianchi groups are $\mathbb{Z}$-points of a $\mathbb{Z}$-group scheme and arithmetic subgroups of $\operatorname{SO}_{1,n+1}(\mathbb{R})^{\circ}$ with their fractional linear action. We report on groups acting on $\mathcal{H}^4$, $\mathcal{H}^5$, and $\mathcal{H}^6$. Agents using Claude Code and OpenAI Codex assisted with proofreading, Lean formalization, and figures; their use is described in the manuscript.

==> tikz/new-mobius-data.tex <==
\def\flagid{(0.450,0.350) -- (0.450,0.370) -- (0.450,0.390) -- (0.450,0.410) -- (0.450,0.430) -- (0.450,0.450) -- (0.450,0.470) -- (0.450,0.490) -- (0.450,0.510) -- (0.450,0.530) -- (0.450,0.550) -- (0.450,0.570) -- (0.450,0.590) -- (0.450,0.610) -- (0.450,0.630) -- (0.450,0.650) -- (0.450,0.670) -- (0.450,0.690) -- (0.450,0.710) -- (0.450,0.730) -- (0.450,0.750) -- (0.450,0.770) -- (0.450,0.790) -- (0.450,0.810) -- (0.450,0.830) -- (0.450,0.850) -- (0.450,0.870) -- (0.450,0.890) -- (0.450,0.910) -- (0.450,0.930) -- (0.450,0.950) -- (0.450,0.970) -- (0.450,0.990) -- (0.450,1.010) -- (0.450,1.030) -- (0.450,1.050) -- (0.450,1.070) -- (0.450,1.090) -- (0.450,1.110) -- (0.450,1.130) -- (0.450,1.150) -- (0.463,1.150) -- (0.475,1.150) -- (0.487,1.150) -- (0.500,1.150) -- (0.512,1.150) -- (0.525,1.150) -- (0.537,1.150) -- (0.550,1.150) -- (0.562,1.150) -- (0.575,1.150) -- (0.588,1.150) -- (0.600,1.150) -- (0.613,1.150) -- (0.625,1.150) -- (0.637,1.150) -- (0.650,1.150) -- (0.662,1.150) -- (0.675,1.150) -- (0.688,1.150) -- (0.700,1.150) -- (0.712,1.150) -- (0.725,1.150) -- (0.738,1.150) -- (0.750,1.150) -- (0.762,1.150) -- (0.775,1.150) -- (0.787,1.150) -- (0.800,1.150) -- (0.812,1.150) -- (0.825,1.150) -- (0.837,1.150) -- (0.850,1.150) -- (0.862,1.150) -- (0.875,1.150) -- (0.887,1.150) -- (0.900,1.150) -- (0.912,1.150) -- (0.925,1.150) -- (0.938,1.150) -- (0.950,1.150) -- (0.950,1.146) -- (0.950,1.142) -- (0.950,1.139) -- (0.950,1.135) -- (0.950,1.131) -- (0.950,1.127) -- (0.950,1.124) -- (0.950,1.120) -- (0.950,1.116) -- (0.950,1.112) -- (0.950,1.109) -- (0.950,1.105) -- (0.950,1.101) -- (0.950,1.097) -- (0.950,1.094) -- (0.950,1.090) -- (0.950,1.086) -- (0.950,1.083) -- (0.950,1.079) -- (0.950,1.075) -- (0.950,1.071) -- (0.950,1.067) -- (0.950,1.064) -- (0.950,1.060) -- (0.950,1.056) -- (0.950,1.052) -- (0.950,1.049) -- (0.950,1.045) -- (0.950,1.041) -- (0.950,1.038) -- (0.950,1.034) -- (0.950,1.030) -- (0.950,1.026) -- (0.950,1.022) -- (0.950,1.019) -- (0.950,1.015) -- (0.950,1.011) -- (0.950,1.008) -- (0.950,1.004) -- (0.950,1.000) -- (0.941,1.000) -- (0.932,1.000) -- (0.924,1.000) -- (0.915,1.000) -- (0.906,1.000) -- (0.897,1.000) -- (0.889,1.000) -- (0.880,1.000) -- (0.871,1.000) -- (0.862,1.000) -- (0.854,1.000) -- (0.845,1.000) -- (0.836,1.000) -- (0.828,1.000) -- (0.819,1.000) -- (0.810,1.000) -- (0.801,1.000) -- (0.792,1.000) -- (0.784,1.000) -- (0.775,1.000) -- (0.766,1.000) -- (0.757,1.000) -- (0.749,1.000) -- (0.740,1.000) -- (0.731,1.000) -- (0.722,1.000) -- (0.714,1.000) -- (0.705,1.000) -- (0.696,1.000) -- (0.688,1.000) -- (0.679,1.000) -- (0.670,1.000) -- (0.661,1.000) -- (0.652,1.000) -- (0.644,1.000) -- (0.635,1.000) -- (0.626,1.000) -- (0.617,1.000) -- (0.609,1.000) -- (0.600,1.000) -- (0.600,0.995) -- (0.600,0.990) -- (0.600,0.985) -- (0.600,0.980) -- (0.600,0.975) -- (0.600,0.970) -- (0.600,0.965) -- (0.600,0.960) -- (0.600,0.955) -- (0.600,0.950) -- (0.600,0.945) -- (0.600,0.940) -- (0.600,0.935) -- (0.600,0.930) -- (0.600,0.925) -- (0.600,0.920) -- (0.600,0.915) -- (0.600,0.910) -- (0.600,0.905) -- (0.600,0.900) -- (0.600,0.895) -- (0.600,0.890) -- (0.600,0.885) -- (0.600,0.880) -- (0.600,0.875) -- (0.600,0.870) -- (0.600,0.865) -- (0.600,0.860) -- (0.600,0.855) -- (0.600,0.850) -- (0.600,0.845) -- (0.600,0.840) -- (0.600,0.835) -- (0.600,0.830) -- (0.600,0.825) -- (0.600,0.820) -- (0.600,0.815) -- (0.600,0.810) -- (0.600,0.805) -- (0.600,0.800) -- (0.606,0.800) -- (0.612,0.800) -- (0.619,0.800) -- (0.625,0.800) -- (0.631,0.800) -- (0.637,0.800) -- (0.644,0.800) -- (0.650,0.800) -- (0.656,0.800) -- (0.662,0.800) -- (0.669,0.800) -- (0.675,0.800) -- (0.681,0.800) -- (0.688,0.800) -- (0.694,0.800) -- (0.700,0.800) -- (0.706,0.800) -- (0.713,0.800) -- (0.719,0.800) -- (0.725,0.800) -- (0.731,0.800) -- (0.738,0.800) -- (0.744,0.800) -- (0.750,0.800) -- (0.756,0.800) -- (0.762,0.800) -- (0.769,0.800) -- (0.775,0.800) -- (0.781,0.800) -- (0.787,0.800) -- (0.794,0.800) -- (0.800,0.800) -- (0.806,0.800) -- (0.812,0.800) -- (0.819,0.800) -- (0.825,0.800) -- (0.831,0.800) -- (0.837,0.800) -- (0.844,0.800) -- (0.850,0.800) -- (0.850,0.796) -- (0.850,0.793) -- (0.850,0.789) -- (0.850,0.785) -- (0.850,0.781) -- (0.850,0.778) -- (0.850,0.774) -- (0.850,0.770) -- (0.850,0.766) -- (0.850,0.763) -- (0.850,0.759) -- (0.850,0.755) -- (0.850,0.751) -- (0.850,0.748) -- (0.850,0.744) -- (0.850,0.740) -- (0.850,0.736) -- (0.850,0.733) -- (0.850,0.729) -- (0.850,0.725) -- (0.850,0.721) -- (0.850,0.718) -- (0.850,0.714) -- (0.850,0.710) -- (0.850,0.706) -- (0.850,0.703) -- (0.850,0.699) -- (0.850,0.695) -- (0.850,0.691) -- (0.850,0.688) -- (0.850,0.684) -- (0.850,0.680) -- (0.850,0.676) -- (0.850,0.673) -- (0.850,0.669) -- (0.850,0.665) -- (0.850,0.661) -- (0.850,0.657) -- (0.850,0.654) -- (0.850,0.650) -- (0.844,0.650) -- (0.838,0.650) -- (0.831,0.650) -- (0.825,0.650) -- (0.819,0.650) -- (0.812,0.650) -- (0.806,0.650) -- (0.800,0.650) -- (0.794,0.650) -- (0.787,0.650) -- (0.781,0.650) -- (0.775,0.650) -- (0.769,0.650) -- (0.762,0.650) -- (0.756,0.650) -- (0.750,0.650) -- (0.744,0.650) -- (0.737,0.650) -- (0.731,0.650) -- (0.725,0.650) -- (0.719,0.650) -- (0.712,0.650) -- (0.706,0.650) -- (0.700,0.650) -- (0.694,0.650) -- (0.688,0.650) -- (0.681,0.650) -- (0.675,0.650) -- (0.669,0.650) -- (0.662,0.650) -- (0.656,0.650) -- (0.650,0.650) -- (0.644,0.650) -- (0.637,0.650) -- (0.631,0.650) -- (0.625,0.650) -- (0.619,0.650) -- (0.613,0.650) -- (0.606,0.650) -- (0.600,0.650) -- (0.600,0.643) -- (0.600,0.635) -- (0.600,0.628) -- (0.600,0.620) -- (0.600,0.613) -- (0.600,0.605) -- (0.600,0.598) -- (0.600,0.590) -- (0.600,0.583) -- (0.600,0.575) -- (0.600,0.568) -- (0.600,0.560) -- (0.600,0.552) -- (0.600,0.545) -- (0.600,0.537) -- (0.600,0.530) -- (0.600,0.522) -- (0.600,0.515) -- (0.600,0.508) -- (0.600,0.500) -- (0.600,0.492) -- (0.600,0.485) -- (0.600,0.477) -- (0.600,0.470) -- (0.600,0.463) -- (0.600,0.455) -- (0.600,0.448) -- (0.600,0.440) -- (0.600,0.432) -- (0.600,0.425) -- (0.600,0.417) -- (0.600,0.410) -- (0.600,0.402) -- (0.600,0.395) -- (0.600,0.387) -- (0.600,0.380) -- (0.600,0.372) -- (0.600,0.365) -- (0.600,0.357) -- (0.600,0.350) -- (0.596,0.350) -- (0.593,0.350) -- (0.589,0.350) -- (0.585,0.350) -- (0.581,0.350) -- (0.578,0.350) -- (0.574,0.350) -- (0.570,0.350) -- (0.566,0.350) -- (0.562,0.350) -- (0.559,0.350) -- (0.555,0.350) -- (0.551,0.350) -- (0.547,0.350) -- (0.544,0.350) -- (0.540,0.350) -- (0.536,0.350) -- (0.532,0.350) -- (0.529,0.350) -- (0.525,0.350) -- (0.521,0.350) -- (0.517,0.350) -- (0.514,0.350) -- (0.510,0.350) -- (0.506,0.350) -- (0.502,0.350) -- (0.499,0.350) -- (0.495,0.350) -- (0.491,0.350) -- (0.487,0.350) -- (0.484,0.350) -- (0.480,0.350) -- (0.476,0.350) -- (0.473,0.350) -- (0.469,0.350) -- (0.465,0.350) -- (0.461,0.350) -- (0.458,0.350) -- (0.454,0.350) -- cycle}
\def\flagtrans{(-0.750,-0.050) -- (-0.750,-0.030) -- (-0.750,-0.010) -- (-0.750,0.010) -- (-0.750,0.030) -- (-0.750,0.050) -- (-0.750,0.070) -- (-0.750,0.090) -- (-0.750,0.110) -- (-0.750,0.130) -- (-0.750,0.150) -- (-0.750,0.170) -- (-0.750,0.190) -- (-0.750,0.210) -- (-0.750,0.230) -- (-0.750,0.250) -- (-0.750,0.270) -- (-0.750,0.290) -- (-0.750,0.310) -- (-0.750,0.330) -- (-0.750,0.350) -- (-0.750,0.370) -- (-0.750,0.390) -- (-0.750,0.410) -- (-0.750,0.430) -- (-0.750,0.450) -- (-0.750,0.470) -- (-0.750,0.490) -- (-0.750,0.510) -- (-0.750,0.530) -- (-0.750,0.550) -- (-0.750,0.570) -- (-0.750,0.590) -- (-0.750,0.610) -- (-0.750,0.630) -- (-0.750,0.650) -- (-0.750,0.670) -- (-0.750,0.690) -- (-0.750,0.710) -- (-0.750,0.730) -- (-0.750,0.750) -- (-0.737,0.750) -- (-0.725,0.750) -- (-0.712,0.750) -- (-0.700,0.750) -- (-0.688,0.750) -- (-0.675,0.750) -- (-0.662,0.750) -- (-0.650,0.750) -- (-0.637,0.750) -- (-0.625,0.750) -- (-0.612,0.750) -- (-0.600,0.750) -- (-0.587,0.750) -- (-0.575,0.750) -- (-0.562,0.750) -- (-0.550,0.750) -- (-0.537,0.750) -- (-0.525,0.750) -- (-0.512,0.750) -- (-0.500,0.750) -- (-0.488,0.750) -- (-0.475,0.750) -- (-0.462,0.750) -- (-0.450,0.750) -- (-0.438,0.750) -- (-0.425,0.750) -- (-0.412,0.750) -- (-0.400,0.750) -- (-0.387,0.750) -- (-0.375,0.750) -- (-0.363,0.750) -- (-0.350,0.750) -- (-0.338,0.750) -- (-0.325,0.750) -- (-0.312,0.750) -- (-0.300,0.750) -- (-0.288,0.750) -- (-0.275,0.750) -- (-0.262,0.750) -- (-0.250,0.750) -- (-0.250,0.746) -- (-0.250,0.742) -- (-0.250,0.739) -- (-0.250,0.735) -- (-0.250,0.731) -- (-0.250,0.727) -- (-0.250,0.724) -- (-0.250,0.720) -- (-0.250,0.716) -- (-0.250,0.712) -- (-0.250,0.709) -- (-0.250,0.705) -- (-0.250,0.701) -- (-0.250,0.697) -- (-0.250,0.694) -- (-0.250,0.690) -- (-0.250,0.686) -- (-0.250,0.682) -- (-0.250,0.679) -- (-0.250,0.675) -- (-0.250,0.671) -- (-0.250,0.667) -- (-0.250,0.664) -- (-0.250,0.660) -- (-0.250,0.656) -- (-0.250,0.652) -- (-0.250,0.649) -- (-0.250,0.645) -- (-0.250,0.641) -- (-0.250,0.638) -- (-0.250,0.634) -- (-0.250,0.630) -- (-0.250,0.626) -- (-0.250,0.622) -- (-0.250,0.619) -- (-0.250,0.615) -- (-0.250,0.611) -- (-0.250,0.608) -- (-0.250,0.604) -- (-0.250,0.600) -- (-0.259,0.600) -- (-0.267,0.600) -- (-0.276,0.600) -- (-0.285,0.600) -- (-0.294,0.600) -- (-0.302,0.600) -- (-0.311,0.600) -- (-0.320,0.600) -- (-0.329,0.600) -- (-0.338,0.600) -- (-0.346,0.600) -- (-0.355,0.600) -- (-0.364,0.600) -- (-0.372,0.600) -- (-0.381,0.600) -- (-0.390,0.600) -- (-0.399,0.600) -- (-0.407,0.600) -- (-0.416,0.600) -- (-0.425,0.600) -- (-0.434,0.600) -- (-0.443,0.600) -- (-0.451,0.600) -- (-0.460,0.600) -- (-0.469,0.600) -- (-0.478,0.600) -- (-0.486,0.600) -- (-0.495,0.600) -- (-0.504,0.600) -- (-0.512,0.600) -- (-0.521,0.600) -- (-0.530,0.600) -- (-0.539,0.600) -- (-0.547,0.600) -- (-0.556,0.600) -- (-0.565,0.600) -- (-0.574,0.600) -- (-0.583,0.600) -- (-0.591,0.600) -- (-0.600,0.600) -- (-0.600,0.595) -- (-0.600,0.590) -- (-0.600,0.585) -- (-0.600,0.580) -- (-0.600,0.575) -- (-0.600,0.570) -- (-0.600,0.565) -- (-0.600,0.560) -- (-0.600,0.555) -- (-0.600,0.550) -- (-0.600,0.545) -- (-0.600,0.540) -- (-0.600,0.535) -- (-0.600,0.530) -- (-0.600,0.525) -- (-0.600,0.520) -- (-0.600,0.515) -- (-0.600,0.510) -- (-0.600,0.505) -- (-0.600,0.500) -- (-0.600,0.495) -- (-0.600,0.490) -- (-0.600,0.485) -- (-0.600,0.480) -- (-0.600,0.475) -- (-0.600,0.470) -- (-0.600,0.465) -- (-0.600,0.460) -- (-0.600,0.455) -- (-0.600,0.450) -- (-0.600,0.445) -- (-0.600,0.440) -- (-0.600,0.435) -- (-0.600,0.430) -- (-0.600,0.425) -- (-0.600,0.420) -- (-0.600,0.415) -- (-0.600,0.410) -- (-0.600,0.405) -- (-0.600,0.400) -- (-0.594,0.400) -- (-0.588,0.400) -- (-0.581,0.400) -- (-0.575,0.400) -- (-0.569,0.400) -- (-0.562,0.400) -- (-0.556,0.400) -- (-0.550,0.400) -- (-0.544,0.400) -- (-0.537,0.400) -- (-0.531,0.400) -- (-0.525,0.400) -- (-0.519,0.400) -- (-0.512,0.400) -- (-0.506,0.400) -- (-0.500,0.400) -- (-0.494,0.400) -- (-0.487,0.400) -- (-0.481,0.400) -- (-0.475,0.400) -- (-0.469,0.400) -- (-0.462,0.400) -- (-0.456,0.400) -- (-0.450,0.400) -- (-0.444,0.400) -- (-0.438,0.400) -- (-0.431,0.400) -- (-0.425,0.400) -- (-0.419,0.400) -- (-0.412,0.400) -- (-0.406,0.400) -- (-0.400,0.400) -- (-0.394,0.400) -- (-0.387,0.400) -- (-0.381,0.400) -- (-0.375,0.400) -- (-0.369,0.400) -- (-0.363,0.400) -- (-0.356,0.400) -- (-0.350,0.400) -- (-0.350,0.396) -- (-0.350,0.393) -- (-0.350,0.389) -- (-0.350,0.385) -- (-0.350,0.381) -- (-0.350,0.378) -- (-0.350,0.374) -- (-0.350,0.370) -- (-0.350,0.366) -- (-0.350,0.363) -- (-0.350,0.359) -- (-0.350,0.355) -- (-0.350,0.351) -- (-0.350,0.348) -- (-0.350,0.344) -- (-0.350,0.340) -- (-0.350,0.336) -- (-0.350,0.333) -- (-0.350,0.329) -- (-0.350,0.325) -- (-0.350,0.321) -- (-0.350,0.318) -- (-0.350,0.314) -- (-0.350,0.310) -- (-0.350,0.306) -- (-0.350,0.302) -- (-0.350,0.299) -- (-0.350,0.295) -- (-0.350,0.291) -- (-0.350,0.287) -- (-0.350,0.284) -- (-0.350,0.280) -- (-0.350,0.276) -- (-0.350,0.273) -- (-0.350,0.269) -- (-0.350,0.265) -- (-0.350,0.261) -- (-0.350,0.257) -- (-0.350,0.254) -- (-0.350,0.250) -- (-0.356,0.250) -- (-0.362,0.250) -- (-0.369,0.250) -- (-0.375,0.250) -- (-0.381,0.250) -- (-0.387,0.250) -- (-0.394,0.250) -- (-0.400,0.250) -- (-0.406,0.250) -- (-0.412,0.250) -- (-0.419,0.250) -- (-0.425,0.250) -- (-0.431,0.250) -- (-0.438,0.250) -- (-0.444,0.250) -- (-0.450,0.250) -- (-0.456,0.250) -- (-0.463,0.250) -- (-0.469,0.250) -- (-0.475,0.250) -- (-0.481,0.250) -- (-0.488,0.250) -- (-0.494,0.250) -- (-0.500,0.250) -- (-0.506,0.250) -- (-0.512,0.250) -- (-0.519,0.250) -- (-0.525,0.250) -- (-0.531,0.250) -- (-0.537,0.250) -- (-0.544,0.250) -- (-0.550,0.250) -- (-0.556,0.250) -- (-0.562,0.250) -- (-0.569,0.250) -- (-0.575,0.250) -- (-0.581,0.250) -- (-0.587,0.250) -- (-0.594,0.250) -- (-0.600,0.250) -- (-0.600,0.243) -- (-0.600,0.235) -- (-0.600,0.228) -- (-0.600,0.220) -- (-0.600,0.213) -- (-0.600,0.205) -- (-0.600,0.198) -- (-0.600,0.190) -- (-0.600,0.182) -- (-0.600,0.175) -- (-0.600,0.167) -- (-0.600,0.160) -- (-0.600,0.152) -- (-0.600,0.145) -- (-0.600,0.137) -- (-0.600,0.130) -- (-0.600,0.122) -- (-0.600,0.115) -- (-0.600,0.108) -- (-0.600,0.100) -- (-0.600,0.092) -- (-0.600,0.085) -- (-0.600,0.077) -- (-0.600,0.070) -- (-0.600,0.062) -- (-0.600,0.055) -- (-0.600,0.047) -- (-0.600,0.040) -- (-0.600,0.032) -- (-0.600,0.025) -- (-0.600,0.017) -- (-0.600,0.010) -- (-0.600,0.002) -- (-0.600,-0.005) -- (-0.600,-0.013) -- (-0.600,-0.020) -- (-0.600,-0.028) -- (-0.600,-0.035) -- (-0.600,-0.043) -- (-0.600,-0.050) -- (-0.604,-0.050) -- (-0.607,-0.050) -- (-0.611,-0.050) -- (-0.615,-0.050) -- (-0.619,-0.050) -- (-0.622,-0.050) -- (-0.626,-0.050) -- (-0.630,-0.050) -- (-0.634,-0.050) -- (-0.637,-0.050) -- (-0.641,-0.050) -- (-0.645,-0.050) -- (-0.649,-0.050) -- (-0.652,-0.050) -- (-0.656,-0.050) -- (-0.660,-0.050) -- (-0.664,-0.050) -- (-0.667,-0.050) -- (-0.671,-0.050) -- (-0.675,-0.050) -- (-0.679,-0.050) -- (-0.682,-0.050) -- (-0.686,-0.050) -- (-0.690,-0.050) -- (-0.694,-0.050) -- (-0.698,-0.050) -- (-0.701,-0.050) -- (-0.705,-0.050) -- (-0.709,-0.050) -- (-0.712,-0.050) -- (-0.716,-0.050) -- (-0.720,-0.050) -- (-0.724,-0.050) -- (-0.727,-0.050) -- (-0.731,-0.050) -- (-0.735,-0.050) -- (-0.739,-0.050) -- (-0.742,-0.050) -- (-0.746,-0.050) -- cycle}
\def\flaginv{(-1.385,1.077) -- (-1.326,1.090) -- (-1.269,1.100) -- (-1.214,1.106) -- (-1.162,1.110) -- (-1.111,1.111) -- (-1.063,1.110) -- (-1.017,1.107) -- (-0.973,1.102) -- (-0.931,1.096) -- (-0.891,1.089) -- (-0.853,1.081) -- (-0.817,1.072) -- (-0.783,1.062) -- (-0.751,1.051) -- (-0.720,1.040) -- (-0.691,1.029) -- (-0.663,1.017) -- (-0.637,1.005) -- (-0.612,0.993) -- (-0.588,0.980) -- (-0.566,0.968) -- (-0.544,0.956) -- (-0.524,0.943) -- (-0.505,0.931) -- (-0.486,0.919) -- (-0.469,0.907) -- (-0.452,0.895) -- (-0.437,0.883) -- (-0.422,0.871) -- (-0.407,0.860) -- (-0.394,0.848) -- (-0.381,0.837) -- (-0.368,0.826) -- (-0.356,0.815) -- (-0.345,0.805) -- (-0.334,0.794) -- (-0.324,0.784) -- (-0.314,0.774) -- (-0.304,0.764) -- (-0.295,0.754) -- (-0.301,0.748) -- (-0.307,0.743) -- (-0.312,0.737) -- (-0.318,0.731) -- (-0.323,0.725) -- (-0.329,0.720) -- (-0.334,0.714) -- (-0.338,0.708) -- (-0.343,0.702) -- (-0.348,0.696) -- (-0.352,0.690) -- (-0.357,0.684) -- (-0.361,0.677) -- (-0.365,0.671) -- (-0.369,0.665) -- (-0.372,0.659) -- (-0.376,0.653) -- (-0.380,0.647) -- (-0.383,0.641) -- (-0.386,0.634) -- (-0.389,0.628) -- (-0.392,0.622) -- (-0.395,0.616) -- (-0.398,0.610) -- (-0.400,0.604) -- (-0.403,0.598) -- (-0.405,0.592) -- (-0.408,0.586) -- (-0.410,0.580) -- (-0.412,0.574) -- (-0.414,0.568) -- (-0.416,0.562) -- (-0.417,0.557) -- (-0.419,0.551) -- (-0.421,0.545) -- (-0.422,0.539) -- (-0.423,0.534) -- (-0.425,0.528) -- (-0.426,0.522) -- (-0.427,0.517) -- (-0.429,0.517) -- (-0.430,0.517) -- (-0.432,0.518) -- (-0.434,0.518) -- (-0.435,0.518) -- (-0.437,0.519) -- (-0.439,0.519) -- (-0.440,0.519) -- (-0.442,0.520) -- (-0.444,0.520) -- (-0.446,0.520) -- (-0.447,0.520) -- (-0.449,0.521) -- (-0.451,0.521) -- (-0.453,0.521) -- (-0.454,0.521) -- (-0.456,0.522) -- (-0.458,0.522) -- (-0.460,0.522) -- (-0.462,0.522) -- (-0.463,0.523) -- (-0.465,0.523) -- (-0.467,0.523) -- (-0.469,0.523) -- (-0.471,0.523) -- (-0.473,0.524) -- (-0.474,0.524) -- (-0.476,0.524) -- (-0.478,0.524) -- (-0.480,0.524) -- (-0.482,0.524) -- (-0.484,0.525) -- (-0.486,0.525) -- (-0.488,0.525) -- (-0.490,0.525) -- (-0.492,0.525) -- (-0.493,0.525) -- (-0.495,0.525) -- (-0.497,0.526) -- (-0.499,0.526) -- (-0.499,0.530) -- (-0.499,0.535) -- (-0.498,0.540) -- (-0.498,0.544) -- (-0.498,0.549) -- (-0.497,0.554) -- (-0.497,0.559) -- (-0.496,0.564) -- (-0.495,0.568) -- (-0.495,0.573) -- (-0.494,0.578) -- (-0.493,0.583) -- (-0.492,0.588) -- (-0.491,0.594) -- (-0.490,0.599) -- (-0.489,0.604) -- (-0.488,0.609) -- (-0.487,0.614) -- (-0.486,0.619) -- (-0.484,0.625) -- (-0.483,0.630) -- (-0.481,0.635) -- (-0.480,0.641) -- (-0.478,0.646) -- (-0.476,0.652) -- (-0.475,0.657) -- (-0.473,0.662) -- (-0.471,0.668) -- (-0.469,0.674) -- (-0.467,0.679) -- (-0.465,0.685) -- (-0.462,0.690) -- (-0.460,0.696) -- (-0.458,0.701) -- (-0.455,0.707) -- (-0.453,0.713) -- (-0.450,0.718) -- (-0.447,0.724) -- (-0.444,0.730) -- (-0.441,0.735) -- (-0.444,0.737) -- (-0.448,0.739) -- (-0.451,0.740) -- (-0.454,0.742) -- (-0.458,0.744) -- (-0.461,0.746) -- (-0.465,0.747) -- (-0.468,0.749) -- (-0.472,0.751) -- (-0.475,0.752) -- (-0.479,0.754) -- (-0.482,0.756) -- (-0.486,0.758) -- (-0.490,0.759) -- (-0.494,0.761) -- (-0.497,0.763) -- (-0.501,0.764) -- (-0.505,0.766) -- (-0.509,0.768) -- (-0.513,0.769) -- (-0.517,0.771) -- (-0.521,0.773) -- (-0.525,0.774) -- (-0.529,0.776) -- (-0.533,0.777) -- (-0.537,0.779) -- (-0.541,0.781) -- (-0.546,0.782) -- (-0.550,0.784) -- (-0.554,0.785) -- (-0.559,0.787) -- (-0.563,0.788) -- (-0.568,0.790) -- (-0.572,0.791) -- (-0.577,0.793) -- (-0.581,0.794) -- (-0.586,0.796) -- (-0.590,0.797) -- (-0.595,0.799) -- (-0.600,0.800) -- (-0.602,0.794) -- (-0.603,0.788) -- (-0.605,0.782) -- (-0.606,0.776) -- (-0.608,0.770) -- (-0.609,0.765) -- (-0.611,0.759) -- (-0.612,0.753) -- (-0.613,0.747) -- (-0.614,0.741) -- (-0.615,0.736) -- (-0.616,0.730) -- (-0.617,0.725) -- (-0.618,0.719) -- (-0.619,0.713) -- (-0.619,0.708) -- (-0.620,0.703) -- (-0.621,0.697) -- (-0.621,0.692) -- (-0.622,0.686) -- (-0.622,0.681) -- (-0.623,0.676) -- (-0.623,0.670) -- (-0.624,0.665) -- (-0.624,0.660) -- (-0.624,0.655) -- (-0.625,0.650) -- (-0.625,0.645) -- (-0.625,0.640) -- (-0.625,0.635) -- (-0.625,0.630) -- (-0.625,0.625) -- (-0.625,0.620) -- (-0.625,0.615) -- (-0.625,0.611) -- (-0.625,0.606) -- (-0.625,0.601) -- (-0.624,0.596) -- (-0.624,0.592) -- (-0.624,0.587) -- (-0.627,0.587) -- (-0.629,0.587) -- (-0.632,0.587) -- (-0.635,0.586) -- (-0.638,0.586) -- (-0.641,0.586) -- (-0.643,0.586) -- (-0.646,0.585) -- (-0.649,0.585) -- (-0.652,0.585) -- (-0.655,0.584) -- (-0.658,0.584) -- (-0.661,0.584) -- (-0.663,0.583) -- (-0.666,0.583) -- (-0.669,0.583) -- (-0.672,0.582) -- (-0.675,0.582) -- (-0.678,0.581) -- (-0.681,0.581) -- (-0.684,0.580) -- (-0.687,0.580) -- (-0.690,0.579) -- (-0.693,0.579) -- (-0.696,0.578) -- (-0.699,0.578) -- (-0.702,0.577) -- (-0.705,0.577) -- (-0.708,0.576) -- (-0.711,0.575) -- (-0.714,0.575) -- (-0.717,0.574) -- (-0.720,0.573) -- (-0.724,0.572) -- (-0.727,0.572) -- (-0.730,0.571) -- (-0.733,0.570) -- (-0.736,0.569) -- (-0.739,0.569) -- (-0.742,0.568) -- (-0.744,0.573) -- (-0.745,0.578) -- (-0.747,0.584) -- (-0.748,0.589) -- (-0.749,0.595) -- (-0.750,0.600) -- (-0.752,0.606) -- (-0.753,0.612) -- (-0.754,0.618) -- (-0.755,0.623) -- (-0.756,0.629) -- (-0.757,0.635) -- (-0.759,0.641) -- (-0.760,0.647) -- (-0.760,0.654) -- (-0.761,0.660) -- (-0.762,0.666) -- (-0.763,0.673) -- (-0.764,0.679) -- (-0.765,0.686) -- (-0.765,0.692) -- (-0.766,0.699) -- (-0.767,0.706) -- (-0.767,0.712) -- (-0.768,0.719) -- (-0.768,0.726) -- (-0.768,0.733) -- (-0.769,0.740) -- (-0.769,0.747) -- (-0.769,0.755) -- (-0.769,0.762) -- (-0.769,0.769) -- (-0.769,0.777) -- (-0.769,0.784) -- (-0.769,0.792) -- (-0.769,0.799) -- (-0.768,0.807) -- (-0.768,0.815) -- (-0.767,0.823) -- (-0.767,0.831) -- (-0.776,0.831) -- (-0.786,0.832) -- (-0.796,0.832) -- (-0.806,0.833) -- (-0.816,0.833) -- (-0.826,0.833) -- (-0.837,0.833) -- (-0.847,0.833) -- (-0.858,0.833) -- (-0.869,0.833) -- (-0.880,0.832) -- (-0.891,0.831) -- (-0.902,0.831) -- (-0.913,0.829) -- (-0.925,0.828) -- (-0.936,0.827) -- (-0.948,0.825) -- (-0.960,0.824) -- (-0.972,0.822) -- (-0.984,0.820) -- (-0.996,0.817) -- (-1.008,0.815) -- (-1.020,0.812) -- (-1.033,0.809) -- (-1.045,0.806) -- (-1.058,0.802) -- (-1.071,0.799) -- (-1.084,0.795) -- (-1.097,0.791) -- (-1.110,0.786) -- (-1.123,0.781) -- (-1.136,0.776) -- (-1.149,0.771) -- (-1.163,0.765) -- (-1.176,0.760) -- (-1.190,0.753) -- (-1.203,0.747) -- (-1.216,0.740) -- (-1.230,0.733) -- (-1.244,0.725) -- (-1.247,0.732) -- (-1.251,0.739) -- (-1.255,0.746) -- (-1.259,0.753) -- (-1.263,0.760) -- (-1.266,0.768) -- (-1.270,0.775) -- (-1.274,0.782) -- (-1.278,0.790) -- (-1.282,0.797) -- (-1.285,0.805) -- (-1.289,0.813) -- (-1.293,0.821) -- (-1.297,0.829) -- (-1.300,0.837) -- (-1.304,0.845) -- (-1.308,0.854) -- (-1.311,0.862) -- (-1.315,0.870) -- (-1.319,0.879) -- (-1.322,0.888) -- (-1.326,0.897) -- (-1.329,0.906) -- (-1.333,0.915) -- (-1.336,0.924) -- (-1.340,0.933) -- (-1.343,0.943) -- (-1.347,0.952) -- (-1.350,0.962) -- (-1.354,0.972) -- (-1.357,0.982) -- (-1.360,0.992) -- (-1.363,1.002) -- (-1.367,1.012) -- (-1.370,1.023) -- (-1.373,1.033) -- (-1.376,1.044) -- (-1.379,1.055) -- (-1.382,1.066) -- cycle}
\def\flagdil{(0.675,0.525) -- (0.675,0.555) -- (0.675,0.585) -- (0.675,0.615) -- (0.675,0.645) -- (0.675,0.675) -- (0.675,0.705) -- (0.675,0.735) -- (0.675,0.765) -- (0.675,0.795) -- (0.675,0.825) -- (0.675,0.855) -- (0.675,0.885) -- (0.675,0.915) -- (0.675,0.945) -- (0.675,0.975) -- (0.675,1.005) -- (0.675,1.035) -- (0.675,1.065) -- (0.675,1.095) -- (0.675,1.125) -- (0.675,1.155) -- (0.675,1.185) -- (0.675,1.215) -- (0.675,1.245) -- (0.675,1.275) -- (0.675,1.305) -- (0.675,1.335) -- (0.675,1.365) -- (0.675,1.395) -- (0.675,1.425) -- (0.675,1.455) -- (0.675,1.485) -- (0.675,1.515) -- (0.675,1.545) -- (0.675,1.575) -- (0.675,1.605) -- (0.675,1.635) -- (0.675,1.665) -- (0.675,1.695) -- (0.675,1.725) -- (0.694,1.725) -- (0.713,1.725) -- (0.731,1.725) -- (0.750,1.725) -- (0.769,1.725) -- (0.788,1.725) -- (0.806,1.725) -- (0.825,1.725) -- (0.844,1.725) -- (0.862,1.725) -- (0.881,1.725) -- (0.900,1.725) -- (0.919,1.725) -- (0.938,1.725) -- (0.956,1.725) -- (0.975,1.725) -- (0.994,1.725) -- (1.012,1.725) -- (1.031,1.725) -- (1.050,1.725) -- (1.069,1.725) -- (1.087,1.725) -- (1.106,1.725) -- (1.125,1.725) -- (1.144,1.725) -- (1.162,1.725) -- (1.181,1.725) -- (1.200,1.725) -- (1.219,1.725) -- (1.237,1.725) -- (1.256,1.725) -- (1.275,1.725) -- (1.294,1.725) -- (1.312,1.725) -- (1.331,1.725) -- (1.350,1.725) -- (1.369,1.725) -- (1.387,1.725) -- (1.406,1.725) -- (1.425,1.725) -- (1.425,1.719) -- (1.425,1.714) -- (1.425,1.708) -- (1.425,1.703) -- (1.425,1.697) -- (1.425,1.691) -- (1.425,1.686) -- (1.425,1.680) -- (1.425,1.674) -- (1.425,1.669) -- (1.425,1.663) -- (1.425,1.657) -- (1.425,1.652) -- (1.425,1.646) -- (1.425,1.641) -- (1.425,1.635) -- (1.425,1.629) -- (1.425,1.624) -- (1.425,1.618) -- (1.425,1.612) -- (1.425,1.607) -- (1.425,1.601) -- (1.425,1.596) -- (1.425,1.590) -- (1.425,1.584) -- (1.425,1.579) -- (1.425,1.573) -- (1.425,1.567) -- (1.425,1.562) -- (1.425,1.556) -- (1.425,1.551) -- (1.425,1.545) -- (1.425,1.539) -- (1.425,1.534) -- (1.425,1.528) -- (1.425,1.522) -- (1.425,1.517) -- (1.425,1.511) -- (1.425,1.506) -- (1.425,1.500) -- (1.412,1.500) -- (1.399,1.500) -- (1.386,1.500) -- (1.372,1.500) -- (1.359,1.500) -- (1.346,1.500) -- (1.333,1.500) -- (1.320,1.500) -- (1.307,1.500) -- (1.294,1.500) -- (1.281,1.500) -- (1.268,1.500) -- (1.254,1.500) -- (1.241,1.500) -- (1.228,1.500) -- (1.215,1.500) -- (1.202,1.500) -- (1.189,1.500) -- (1.176,1.500) -- (1.162,1.500) -- (1.149,1.500) -- (1.136,1.500) -- (1.123,1.500) -- (1.110,1.500) -- (1.097,1.500) -- (1.084,1.500) -- (1.071,1.500) -- (1.057,1.500) -- (1.044,1.500) -- (1.031,1.500) -- (1.018,1.500) -- (1.005,1.500) -- (0.992,1.500) -- (0.979,1.500) -- (0.966,1.500) -- (0.953,1.500) -- (0.939,1.500) -- (0.926,1.500) -- (0.913,1.500) -- (0.900,1.500) -- (0.900,1.492) -- (0.900,1.485) -- (0.900,1.478) -- (0.900,1.470) -- (0.900,1.462) -- (0.900,1.455) -- (0.900,1.448) -- (0.900,1.440) -- (0.900,1.432) -- (0.900,1.425) -- (0.900,1.417) -- (0.900,1.410) -- (0.900,1.403) -- (0.900,1.395) -- (0.900,1.388) -- (0.900,1.380) -- (0.900,1.373) -- (0.900,1.365) -- (0.900,1.357) -- (0.900,1.350) -- (0.900,1.343) -- (0.900,1.335) -- (0.900,1.328) -- (0.900,1.320) -- (0.900,1.312) -- (0.900,1.305) -- (0.900,1.297) -- (0.900,1.290) -- (0.900,1.282) -- (0.900,1.275) -- (0.900,1.268) -- (0.900,1.260) -- (0.900,1.252) -- (0.900,1.245) -- (0.900,1.238) -- (0.900,1.230) -- (0.900,1.223) -- (0.900,1.215) -- (0.900,1.208) -- (0.900,1.200) -- (0.909,1.200) -- (0.919,1.200) -- (0.928,1.200) -- (0.938,1.200) -- (0.947,1.200) -- (0.956,1.200) -- (0.966,1.200) -- (0.975,1.200) -- (0.984,1.200) -- (0.994,1.200) -- (1.003,1.200) -- (1.012,1.200) -- (1.022,1.200) -- (1.031,1.200) -- (1.041,1.200) -- (1.050,1.200) -- (1.059,1.200) -- (1.069,1.200) -- (1.078,1.200) -- (1.087,1.200) -- (1.097,1.200) -- (1.106,1.200) -- (1.116,1.200) -- (1.125,1.200) -- (1.134,1.200) -- (1.144,1.200) -- (1.153,1.200) -- (1.162,1.200) -- (1.172,1.200) -- (1.181,1.200) -- (1.191,1.200) -- (1.200,1.200) -- (1.209,1.200) -- (1.219,1.200) -- (1.228,1.200) -- (1.237,1.200) -- (1.247,1.200) -- (1.256,1.200) -- (1.266,1.200) -- (1.275,1.200) -- (1.275,1.194) -- (1.275,1.189) -- (1.275,1.183) -- (1.275,1.177) -- (1.275,1.172) -- (1.275,1.166) -- (1.275,1.161) -- (1.275,1.155) -- (1.275,1.149) -- (1.275,1.144) -- (1.275,1.138) -- (1.275,1.133) -- (1.275,1.127) -- (1.275,1.121) -- (1.275,1.116) -- (1.275,1.110) -- (1.275,1.104) -- (1.275,1.099) -- (1.275,1.093) -- (1.275,1.088) -- (1.275,1.082) -- (1.275,1.076) -- (1.275,1.071) -- (1.275,1.065) -- (1.275,1.059) -- (1.275,1.054) -- (1.275,1.048) -- (1.275,1.042) -- (1.275,1.037) -- (1.275,1.031) -- (1.275,1.026) -- (1.275,1.020) -- (1.275,1.014) -- (1.275,1.009) -- (1.275,1.003) -- (1.275,0.998) -- (1.275,0.992) -- (1.275,0.986) -- (1.275,0.981) -- (1.275,0.975) -- (1.266,0.975) -- (1.256,0.975) -- (1.247,0.975) -- (1.237,0.975) -- (1.228,0.975) -- (1.219,0.975) -- (1.209,0.975) -- (1.200,0.975) -- (1.191,0.975) -- (1.181,0.975) -- (1.172,0.975) -- (1.163,0.975) -- (1.153,0.975) -- (1.144,0.975) -- (1.134,0.975) -- (1.125,0.975) -- (1.116,0.975) -- (1.106,0.975) -- (1.097,0.975) -- (1.087,0.975) -- (1.078,0.975) -- (1.069,0.975) -- (1.059,0.975) -- (1.050,0.975) -- (1.041,0.975) -- (1.031,0.975) -- (1.022,0.975) -- (1.013,0.975) -- (1.003,0.975) -- (0.994,0.975) -- (0.984,0.975) -- (0.975,0.975) -- (0.966,0.975) -- (0.956,0.975) -- (0.947,0.975) -- (0.938,0.975) -- (0.928,0.975) -- (0.919,0.975) -- (0.909,0.975) -- (0.900,0.975) -- (0.900,0.964) -- (0.900,0.953) -- (0.900,0.941) -- (0.900,0.930) -- (0.900,0.919) -- (0.900,0.907) -- (0.900,0.896) -- (0.900,0.885) -- (0.900,0.874) -- (0.900,0.862) -- (0.900,0.851) -- (0.900,0.840) -- (0.900,0.829) -- (0.900,0.818) -- (0.900,0.806) -- (0.900,0.795) -- (0.900,0.784) -- (0.900,0.772) -- (0.900,0.761) -- (0.900,0.750) -- (0.900,0.739) -- (0.900,0.728) -- (0.900,0.716) -- (0.900,0.705) -- (0.900,0.694) -- (0.900,0.682) -- (0.900,0.671) -- (0.900,0.660) -- (0.900,0.649) -- (0.900,0.637) -- (0.900,0.626) -- (0.900,0.615) -- (0.900,0.604) -- (0.900,0.593) -- (0.900,0.581) -- (0.900,0.570) -- (0.900,0.559) -- (0.900,0.547) -- (0.900,0.536) -- (0.900,0.525) -- (0.894,0.525) -- (0.889,0.525) -- (0.883,0.525) -- (0.877,0.525) -- (0.872,0.525) -- (0.866,0.525) -- (0.861,0.525) -- (0.855,0.525) -- (0.849,0.525) -- (0.844,0.525) -- (0.838,0.525) -- (0.832,0.525) -- (0.827,0.525) -- (0.821,0.525) -- (0.816,0.525) -- (0.810,0.525) -- (0.804,0.525) -- (0.799,0.525) -- (0.793,0.525) -- (0.788,0.525) -- (0.782,0.525) -- (0.776,0.525) -- (0.771,0.525) -- (0.765,0.525) -- (0.759,0.525) -- (0.754,0.525) -- (0.748,0.525) -- (0.742,0.525) -- (0.737,0.525) -- (0.731,0.525) -- (0.726,0.525) -- (0.720,0.525) -- (0.714,0.525) -- (0.709,0.525) -- (0.703,0.525) -- (0.698,0.525) -- (0.692,0.525) -- (0.686,0.525) -- (0.681,0.525) -- cycle}
\def\flagrot{(-0.078,0.565) -- (-0.095,0.575) -- (-0.113,0.585) -- (-0.130,0.595) -- (-0.147,0.605) -- (-0.165,0.615) -- (-0.182,0.625) -- (-0.199,0.635) -- (-0.217,0.645) -- (-0.234,0.655) -- (-0.251,0.665) -- (-0.269,0.675) -- (-0.286,0.685) -- (-0.303,0.695) -- (-0.321,0.705) -- (-0.338,0.715) -- (-0.355,0.725) -- (-0.373,0.735) -- (-0.390,0.745) -- (-0.407,0.755) -- (-0.425,0.765) -- (-0.442,0.775) -- (-0.459,0.785) -- (-0.476,0.795) -- (-0.494,0.805) -- (-0.511,0.815) -- (-0.528,0.825) -- (-0.546,0.835) -- (-0.563,0.845) -- (-0.580,0.855) -- (-0.598,0.865) -- (-0.615,0.875) -- (-0.632,0.885) -- (-0.650,0.895) -- (-0.667,0.905) -- (-0.684,0.915) -- (-0.702,0.925) -- (-0.719,0.935) -- (-0.736,0.945) -- (-0.754,0.955) -- (-0.771,0.965) -- (-0.765,0.976) -- (-0.758,0.986) -- (-0.752,0.997) -- (-0.746,1.008) -- (-0.740,1.019) -- (-0.733,1.030) -- (-0.727,1.040) -- (-0.721,1.051) -- (-0.715,1.062) -- (-0.708,1.073) -- (-0.702,1.084) -- (-0.696,1.095) -- (-0.690,1.105) -- (-0.683,1.116) -- (-0.677,1.127) -- (-0.671,1.138) -- (-0.665,1.149) -- (-0.658,1.160) -- (-0.652,1.170) -- (-0.646,1.181) -- (-0.640,1.192) -- (-0.633,1.203) -- (-0.627,1.214) -- (-0.621,1.225) -- (-0.615,1.235) -- (-0.608,1.246) -- (-0.602,1.257) -- (-0.596,1.268) -- (-0.590,1.279) -- (-0.583,1.289) -- (-0.577,1.300) -- (-0.571,1.311) -- (-0.565,1.322) -- (-0.558,1.333) -- (-0.552,1.344) -- (-0.546,1.354) -- (-0.540,1.365) -- (-0.533,1.376) -- (-0.527,1.387) -- (-0.521,1.398) -- (-0.518,1.396) -- (-0.514,1.394) -- (-0.511,1.392) -- (-0.508,1.390) -- (-0.505,1.388) -- (-0.501,1.386) -- (-0.498,1.385) -- (-0.495,1.383) -- (-0.492,1.381) -- (-0.488,1.379) -- (-0.485,1.377) -- (-0.482,1.375) -- (-0.479,1.373) -- (-0.475,1.371) -- (-0.472,1.370) -- (-0.469,1.368) -- (-0.466,1.366) -- (-0.462,1.364) -- (-0.459,1.362) -- (-0.456,1.360) -- (-0.453,1.358) -- (-0.449,1.356) -- (-0.446,1.355) -- (-0.443,1.353) -- (-0.440,1.351) -- (-0.436,1.349) -- (-0.433,1.347) -- (-0.430,1.345) -- (-0.427,1.343) -- (-0.424,1.341) -- (-0.420,1.340) -- (-0.417,1.338) -- (-0.414,1.336) -- (-0.411,1.334) -- (-0.407,1.332) -- (-0.404,1.330) -- (-0.401,1.328) -- (-0.398,1.326) -- (-0.394,1.325) -- (-0.391,1.323) -- (-0.395,1.315) -- (-0.400,1.308) -- (-0.404,1.300) -- (-0.409,1.292) -- (-0.413,1.285) -- (-0.417,1.277) -- (-0.422,1.270) -- (-0.426,1.262) -- (-0.430,1.255) -- (-0.435,1.247) -- (-0.439,1.239) -- (-0.444,1.232) -- (-0.448,1.224) -- (-0.452,1.217) -- (-0.457,1.209) -- (-0.461,1.201) -- (-0.465,1.194) -- (-0.470,1.186) -- (-0.474,1.179) -- (-0.479,1.171) -- (-0.483,1.164) -- (-0.487,1.156) -- (-0.492,1.148) -- (-0.496,1.141) -- (-0.500,1.133) -- (-0.505,1.126) -- (-0.509,1.118) -- (-0.514,1.111) -- (-0.518,1.103) -- (-0.522,1.095) -- (-0.527,1.088) -- (-0.531,1.080) -- (-0.535,1.073) -- (-0.540,1.065) -- (-0.544,1.058) -- (-0.549,1.050) -- (-0.553,1.042) -- (-0.557,1.035) -- (-0.562,1.027) -- (-0.566,1.020) -- (-0.562,1.017) -- (-0.557,1.015) -- (-0.553,1.012) -- (-0.549,1.010) -- (-0.544,1.007) -- (-0.540,1.005) -- (-0.536,1.002) -- (-0.531,1.000) -- (-0.527,0.997) -- (-0.523,0.995) -- (-0.518,0.992) -- (-0.514,0.990) -- (-0.510,0.987) -- (-0.505,0.985) -- (-0.501,0.982) -- (-0.497,0.980) -- (-0.492,0.977) -- (-0.488,0.975) -- (-0.484,0.972) -- (-0.479,0.970) -- (-0.475,0.967) -- (-0.471,0.965) -- (-0.466,0.962) -- (-0.462,0.960) -- (-0.458,0.957) -- (-0.453,0.955) -- (-0.449,0.952) -- (-0.445,0.950) -- (-0.440,0.947) -- (-0.436,0.945) -- (-0.432,0.942) -- (-0.427,0.940) -- (-0.423,0.937) -- (-0.419,0.935) -- (-0.414,0.932) -- (-0.410,0.930) -- (-0.406,0.927) -- (-0.401,0.925) -- (-0.397,0.922) -- (-0.393,0.920) -- (-0.390,0.925) -- (-0.387,0.930) -- (-0.383,0.936) -- (-0.380,0.941) -- (-0.377,0.947) -- (-0.374,0.952) -- (-0.371,0.958) -- (-0.368,0.963) -- (-0.365,0.968) -- (-0.362,0.974) -- (-0.358,0.979) -- (-0.355,0.985) -- (-0.352,0.990) -- (-0.349,0.995) -- (-0.346,1.001) -- (-0.343,1.006) -- (-0.340,1.012) -- (-0.337,1.017) -- (-0.333,1.022) -- (-0.330,1.028) -- (-0.327,1.033) -- (-0.324,1.039) -- (-0.321,1.044) -- (-0.318,1.050) -- (-0.315,1.055) -- (-0.312,1.060) -- (-0.308,1.066) -- (-0.305,1.071) -- (-0.302,1.077) -- (-0.299,1.082) -- (-0.296,1.087) -- (-0.293,1.093) -- (-0.290,1.098) -- (-0.287,1.104) -- (-0.283,1.109) -- (-0.280,1.114) -- (-0.277,1.120) -- (-0.274,1.125) -- (-0.271,1.131) -- (-0.268,1.136) -- (-0.265,1.134) -- (-0.261,1.132) -- (-0.258,1.130) -- (-0.255,1.129) -- (-0.252,1.127) -- (-0.248,1.125) -- (-0.245,1.123) -- (-0.242,1.121) -- (-0.239,1.119) -- (-0.235,1.117) -- (-0.232,1.115) -- (-0.229,1.114) -- (-0.226,1.112) -- (-0.222,1.110) -- (-0.219,1.108) -- (-0.216,1.106) -- (-0.213,1.104) -- (-0.209,1.102) -- (-0.206,1.100) -- (-0.203,1.099) -- (-0.200,1.097) -- (-0.196,1.095) -- (-0.193,1.093) -- (-0.190,1.091) -- (-0.187,1.089) -- (-0.183,1.087) -- (-0.180,1.085) -- (-0.177,1.084) -- (-0.174,1.082) -- (-0.170,1.080) -- (-0.167,1.078) -- (-0.164,1.076) -- (-0.161,1.074) -- (-0.157,1.072) -- (-0.154,1.070) -- (-0.151,1.069) -- (-0.148,1.067) -- (-0.144,1.065) -- (-0.141,1.063) -- (-0.138,1.061) -- (-0.141,1.056) -- (-0.144,1.050) -- (-0.147,1.045) -- (-0.150,1.039) -- (-0.154,1.034) -- (-0.157,1.029) -- (-0.160,1.023) -- (-0.163,1.018) -- (-0.166,1.012) -- (-0.169,1.007) -- (-0.172,1.002) -- (-0.175,0.996) -- (-0.179,0.991) -- (-0.182,0.985) -- (-0.185,0.980) -- (-0.188,0.975) -- (-0.191,0.969) -- (-0.194,0.964) -- (-0.197,0.958) -- (-0.200,0.953) -- (-0.204,0.947) -- (-0.207,0.942) -- (-0.210,0.937) -- (-0.213,0.931) -- (-0.216,0.926) -- (-0.219,0.920) -- (-0.222,0.915) -- (-0.225,0.910) -- (-0.229,0.904) -- (-0.232,0.899) -- (-0.235,0.893) -- (-0.238,0.888) -- (-0.241,0.883) -- (-0.244,0.877) -- (-0.247,0.872) -- (-0.250,0.866) -- (-0.254,0.861) -- (-0.257,0.855) -- (-0.260,0.850) -- (-0.263,0.845) -- (-0.256,0.841) -- (-0.250,0.837) -- (-0.243,0.833) -- (-0.237,0.830) -- (-0.230,0.826) -- (-0.224,0.822) -- (-0.217,0.818) -- (-0.211,0.815) -- (-0.204,0.811) -- (-0.198,0.807) -- (-0.191,0.803) -- (-0.185,0.800) -- (-0.178,0.796) -- (-0.172,0.792) -- (-0.165,0.788) -- (-0.159,0.785) -- (-0.152,0.781) -- (-0.146,0.777) -- (-0.140,0.773) -- (-0.133,0.770) -- (-0.127,0.766) -- (-0.120,0.762) -- (-0.114,0.758) -- (-0.107,0.755) -- (-0.101,0.751) -- (-0.094,0.747) -- (-0.088,0.743) -- (-0.081,0.740) -- (-0.075,0.736) -- (-0.068,0.732) -- (-0.062,0.728) -- (-0.055,0.725) -- (-0.049,0.721) -- (-0.042,0.717) -- (-0.036,0.713) -- (-0.029,0.710) -- (-0.023,0.706) -- (-0.016,0.702) -- (-0.010,0.698) -- (-0.003,0.695) -- (-0.005,0.691) -- (-0.007,0.688) -- (-0.009,0.685) -- (-0.011,0.682) -- (-0.012,0.678) -- (-0.014,0.675) -- (-0.016,0.672) -- (-0.018,0.669) -- (-0.020,0.665) -- (-0.022,0.662) -- (-0.024,0.659) -- (-0.026,0.656) -- (-0.027,0.652) -- (-0.029,0.649) -- (-0.031,0.646) -- (-0.033,0.643) -- (-0.035,0.639) -- (-0.037,0.636) -- (-0.039,0.633) -- (-0.041,0.630) -- (-0.042,0.626) -- (-0.044,0.623) -- (-0.046,0.620) -- (-0.048,0.617) -- (-0.050,0.613) -- (-0.052,0.610) -- (-0.054,0.607) -- (-0.056,0.604) -- (-0.057,0.600) -- (-0.059,0.597) -- (-0.061,0.594) -- (-0.063,0.591) -- (-0.065,0.587) -- (-0.067,0.584) -- (-0.069,0.581) -- (-0.071,0.578) -- (-0.072,0.574) -- (-0.074,0.571) -- (-0.076,0.568) -- cycle}

